Incomplete Pivoted QR-based Dimensionality Reduction

High-dimensional big data appears in many research fields such as image recognition, biology and collaborative filtering. Often, the exploration of such data by classic algorithms is encountered with difficulties due to `curse of dimensionality' phenomenon. Therefore, dimensionality reduction methods are applied to the data prior to its analysis. Many of these methods are based on principal components analysis, which is statistically driven, namely they map the data into a low-dimension subspace that preserves significant statistical properties of the high-dimensional data. As a consequence, such methods do not directly address the geometry of the data, reflected by the mutual distances between multidimensional data point. Thus, operations such as classification, anomaly detection or other machine learning tasks may be affected. This work provides a dictionary-based framework for geometrically driven data analysis that includes dimensionality reduction, out-of-sample extension and anomaly detection. It embeds high-dimensional data in a low-dimensional subspace. This embedding preserves the original high-dimensional geometry of the data up to a user-defined distortion rate. In addition, it identifies a subset of landmark data points that constitute a dictionary for the analyzed dataset. The dictionary enables to have a natural extension of the low-dimensional embedding to out-of-sample data points, which gives rise to a distortion-based criterion for anomaly detection. The suggested method is demonstrated on synthetic and real-world datasets and achieves good results for classification, anomaly detection and out-of-sample tasks.

==> latex-headers.tex <==
\usepackage[title]{appendix}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{afterpage}
\usepackage{etoolbox}
%\usepackage{footbib}
\usepackage{float}
\usepackage{algorithmic}
\usepackage[lined,boxed,linesnumbered,algoruled,vlined]{algorithm2e}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{epstopdf}
\usepackage{multirow}
\usepackage{xcolor,colortbl}
\usepackage[font={small}]{caption}

\usepackage{geometry}
\geometry{
 a4paper,
 total={210mm,297mm},
 left=20mm,
 right=20mm,
 top=20mm,
 bottom=20mm,
 }

\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{table}{section}

\makeatletter
\renewcommand{\p@subfigure}{\thefigure}
\makeatother

\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\newcommand{\repeatable}[2]{\makeatletter \global\expandafter\def\csname repText@#1\endcsname {#2} \makeatother #2}
\newcommand{\repeatxt}[1]{\makeatletter \expandafter\csname repText@#1\endcsname \makeatother}
\newcommand{\repeathm}[3]{{\renewcommand{\thetheorem}{\ref{#2}}\begin{#1}\repeatxt{#3}\end{#1}}}

\newtoggle{citeInAbstract}
\toggletrue{citeInAbstract}
\newcommand{\abstractcite}[1]{\iftoggle{citeInAbstract}{\footcite{#1}}{}}

\newcommand{\usecrop}[2]
{
	\newlength{\cropwidth}
	\setlength{\cropwidth}{\the\textwidth}
	\addtolength{\cropwidth}{#1}
	\newlength{\cropheight}
	\setlength{\cropheight}{\the\textheight}
	\addtolength{\cropheight}{#2}
	\usepackage[width=\the\cropwidth,height=\the\cropheight,center]{crop}
}

\newcommand{\useauthblk}
{
	\usepackage{authblk}
}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\DeclareMathOperator{\len}{len}
\DeclareMathOperator{\source}{s}
\DeclareMathOperator{\target}{t}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\lpr}{lpr}
\DeclareMathOperator{\tr}{tr}
%\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\rank}{\rho}
\DeclareMathOperator{\tcb}{r}
\newcommand{\nrank}{\rank_{\delta}}
\newcommand{\transpose}[1]{#1^T}
\newcommand{\abs}[1]{\left | #1 \right |}
\newcommand{\absinline}[1]{| #1 |}
\newcommand{\norm}[1]{\left \| #1 \right \|}
\newcommand{\norminline}[1]{\| #1 \|}
\newcommand{\inp}[3]{\langle #1, #2\rangle_{#3}}
\newcommand{\inpil}[3]{\left\langle #1, #2\right\rangle_{#3}}
\newcommand{\Rn}[1]{{\mathbbm{R}^{#1}}}
\newcommand{\ve}{\varepsilon}

\makeatletter
\newcommand{\thickhline}{%
    \noalign {\ifnum 0=`}\fi \hrule height 1pt
    \futurelet \reserved@a \@xhline
}
\newcolumntype{"}{@{\hskip\tabcolsep\vrule width 1pt\hskip\tabcolsep}}
\makeatother

% Notations:
\newcommand{\set}{\mathcal}
\newcommand{\vect}{\mathbf}
\newcommand{\ivect}[2]{{\mathbf{#1}}^{({#2})}}
\newcommand{\iscal}[2]{{#1}_{{#2}}}
\newcommand{\map}{\mathbf}
\newcommand{\submat}[3]{{#1}_{({#2},{#3})}}
\newcommand{\rows}[2]{\submat{{#1}}{{#2}}{:}}
\newcommand{\cols}[2]{\submat{{#1}}{:}{{#2}}}
\newcommand{\ventry}[2]{{\vect{#1}}_{(#2)}}
\newcommand{\mentry}[3]{{#1}_{(#2,#3)}}
\newcommand{\bmu}{\boldsymbol\mu}
\newcommand{\mapi}{\boldsymbol\pi}
\newcommand{\proj}[1]{{\map{W}}_{#1}}
\newcommand{\piproj}[1]{\proj{\mapi([#1])}}
\newcommand{\perproj}[1]{{\proj{#1}^\perp}}
\newcommand{\perpiproj}[1]{{\piproj{#1}^\perp}}
\newcommand{\Wpik}[1]{\set{A}_{\mapi([#1])}}
\newcommand{\perpWpik}[1]{\Wpik{#1}^\perp}
\newcommand{\timel}[2]{{#1}^{(#2)}}




